Physically Accurate Differentiable Inverse Rendering for Radio Frequency Digital Twin

Digital twins, virtual simulated replicas of physical scenes, are transforming system design across industries. However, their potential in radio frequency (RF) systems has been limited by the non-differentiable nature of conventional RF simulators. The visibility of propagation paths causes severe discontinuities, and differentiable rendering techniques from computer graphics cannot easily transfer due to point-source antennas and dominant specular reflections. In this paper, we present RFDT, a physically based differentiable RF simulation framework that enables gradient-based interaction between virtual and physical worlds. RFDT resolves discontinuities with a physically grounded edge-diffraction transition function, and mitigates non-convexity from Fourier-domain processing through a signal domain transform surrogate. Our implementation demonstrates RFDT's ability to accurately reconstruct digital twins from real RF measurements. Moreover, RFDT can augment diverse downstream applications, such as test-time adaptation of machine learning-based RF sensing and physically constrained optimization of communication systems.

==> Appendices/psdr.tex <==



==> Chapter/old_diff_method.tex <==
\subsection{Unbiased Differentiation of Geometric Parameters}
\label{sec:diff_cir}
\xya{In this section, we present our approach to addressing the discontinuity challenge, as categorized into two types in Sec.~\ref{sec:discontinuity}. We first formulate the discontinuous integral in path-space, and then handle geometric edges through reparameterization. We further design a custom ray tracing technique to track view-dependent edges. In addition, edge diffraction, often neglected in graphics but critical for RF applications, is treated as a combination of the two types of discontinuity. 
}

The time-domain CIR, aggregating all the multipath components between the transmitter and receiver, can be represented as:
\begin{equation}
    \small
    h(t) = \int_{-\infty}^{\infty} a(\tau) \delta(t - \tau) e^{j\phi(\tau)} \text{d}\tau,
\label{eq:basic_ht}
\end{equation}
\noindent where $\delta$ is the Dirac delta function.
The corresponding frequency domain CIR can be obtained through the Fourier transform:

\begin{equation}
\small
H(f) = \int_{-\infty}^{\infty} h(t) e^{-j2\theta ft} \text{d}t.
\end{equation}

For further derivation, \textit{we transform Equ.~\eqref{eq:basic_ht} into path space by introducing a measurement contribution function} $f$ representing the amount of RF radiant power carried by the ray tracing paths $x = x_{\text{diffract}}\cup x_{\text{reflect}}$:

\begin{equation}
\small
    h(t) = \int_{\Omega} f(x) \, \text{d}\mu(x), \quad f(x) = x_\alpha \delta(t - x_\tau) e^{jx_\phi},
\label{eq:step1}
\end{equation}

\noindent where \(\Omega := \bigcup_{N=1}^{\infty} \mathcal{M}^{N+1}\) is the path space of all possible propagation paths, with each path \(x\) composed of key points \( (x_0, x_1, \dots, x_N) \) representing path intersection locations like reflection or refraction points. The measure \(d\mu(x)\) is defined as \(d\mu(x) := \prod_{n=0}^{N} dA(x_n)\), 
where \(dA(x_n)\) is the area element at each point \(x_n\), accounting for the geometric properties along the path. \(\mathcal{M}\) denotes the union of all object surfaces in the digital twin (DT) scene. 

Discontinuous integrands arise when a ray experiences occlusion or interacts with geometric edges. Consider an example DT scene with three geometries, as illustrated in Fig.~\ref{fig:path_space}(a). Suppose a parameter $\theta$ controls the translation along the X-axis, the relationship between $\theta$ and the time-delay $\tau$ is shown as a function in Fig.~\ref{fig:path_space}(a). 
The function is discontinuous at the edges of the geometries, leading to incorrect estimation of gradients. 

\subsubsection{Path-Space Differentiation}
To correctly differentiate Equ.~\eqref{eq:step1}, we need to explicitly handle the boundary terms by tracking the speed of change of the domain boundary \wrt the target parameter following the Reynolds Transport Theorem \cite{reynolds1895iv}:

\begin{equation}
\small
\frac{\partial h(t)}{\partial \theta} = \underbrace{\int_{\Omega} \frac{\partial}{\partial \theta} f(x) \, \text{d}\mu(x)}_{\text{Interior}} + \underbrace{\int_{\partial \Omega} g(x) \, \text{d}\dot{\mu}(x)}_{\text{Boundary}},
\end{equation}

\noindent where $\partial \Omega$ is the union of all discontinuity points in the domain $\Omega$. Furthermore, \(\partial \Omega\) can be decomposed into two categories, sharp edges, and silhouette edges, \ie, \(\partial \Omega = \partial \Omega_{sharp} \cup \partial \Omega_{sil}\). 
The interior integral term is continuous \wrt the scene state $\theta$ and can be solved using a conventional automatic differentiation system. The boundary term, however, requires tracking all edges in the scene. A common solution is edge sampling, adopted in differentiable visual rendering and more recently in RF ray tracing \cite{chen2023metawave}. This method is costly, and its complexity increases drastically with scene complexity. Alternatively, biased heuristic approximation methods like those used in Sionna \cite{sionna} introduce biases that cause gradient error accumulation. This error accumulation becomes more pronounced as scene complexity increases, negatively affecting convergence on complex tasks.

\subsubsection{Differentiating Geometric Edges through Reparameterization}
\label{sec:reparam}
To overcome the limitations of edge sampling and biased approximation methods, we first parameterize all the geometries in the scene. 
Following previous studies in optical differentiation, continuum mechanics, and topology, all regular geometrical surfaces $\mathcal{M}$ in the scene can be considered to be deformed from some abstract 2D manifold $\mathcal{B}$, referred to as the \textit{reference surface}, as shown in Fig. \ref{fig:path_space}(b).
The deformations $\mathcal{X}(\cdot, \theta)$ are smooth functions that map reference surfaces $\mathcal{B}$ to regular surfaces $\mathcal{M}$, where $\theta \in \mathbb{R}$ is a controlling parameter. A regular surface controlled by parameter $\theta$ is referred to as an \textit{evolving surface} $\mathcal{M}(\theta)$.

We denote the propagation paths in reference space as \(\Omega_0\) and the boundary of the propagation path as \(\partial \Omega_0\). The key idea of our reparameterization technique is to construct the deformation
$\mathcal{X}$ such that \(\partial \Omega_{sharp} \in \Omega_0\), so that the discontinuity originates from sharp edges can be solved. \textit{This essentially works as a change of variables}. Such mapping $\mathcal{X}$ maps the propagation path $x = (x_0, \dots, x_N)$ to the reference space $p = (p_0, \dots, p_N)$ conditioned on mapping parameter \(\theta\). Applying such reparameterization yields a reformed CIR equation:

\vspace{-10pt}
\begin{align}
\small
h(t) = \int_{\Omega_{0}} \hat{f}(p) \, \text{d}\mu(p), \quad x = \mathcal{X}(p, \theta), \textrm{where}\\
    \hat{f}(p) = f(x) \prod_{n=0}^{N} J(p_n, \theta), \quad J(\mathbf{p}, \theta) := \left\| \frac{\text{d}A(\mathbf{x})}{\text{d}A(\mathbf{p})} \right\|,
\end{align}

\noindent and $J(\mathbf{p}, \theta)$ is the Jacobian matrix from the reparameterization. To this end, the final form of the path-space integral becomes:

\vspace{-10pt}
\begin{equation}
\small
\frac{\partial h(t)}{\partial \theta} = 
\underbrace{
\int_{\Omega_0} \frac{\partial}{\partial \theta} \hat{f}(p) \, \text{d}\mu(p)
}_{\text{Interior}}
+ 
\underbrace{
\int_{\partial \Omega_0} \hat{f}(p) V_{\partial}(p_K) \, \text{d}\dot{\mu}(p),
}_{\text{Boundary}}
\label{eq:reparameter_integral}
\end{equation}

\noindent where $\Omega_0$ is the propagation paths in reference space and $\partial\Omega_0$ is the boundary of the propagation path space.

\textit{The reparameterization essentially transforms sharp edges in regular surface \(\mathcal{M}\) to interior points in the reference surface \(\mathcal{B}\)}. Therefore, it resolves the discontinuity due to sharp edges. The remaining boundary term in Equ.~\eqref{eq:reparameter_integral} originates from the discontinuity due to view-dependent edges. Within the boundary term, $\hat{f}(p)$ represents the path contribution function. It integrates over the space of boundary paths $\partial\Omega$, where each path $p_K = (p_0, \ldots, p_N)$ contains a vertex $p_K$ situated precisely on a ``visibility'' boundary, defined as $p_K \in \Delta\mathcal{B}(p_{K-1})$. The function $V_\partial(p_K) = n_\partial(p_K) \cdot \frac{dp_K}{d\theta}$ quantifies the rate at which this boundary shifts \wrt scene state $\theta$, effectively measuring the sensitivity of RF signal occlusion. Here, $n_\partial(p_K)$ denotes the unit normal of the visibility boundary. 
Furthermore, we define the boundary segment caused by silhouette edges as the two-point-path pointing to a visibility boundary:
$(p_{K-1}, p_K) \in \mathcal{B}\times\Delta\mathcal{B}(p_{K-1}).$
    
\subsubsection{Differentiating View-dependent Edges}
\label{sec:view_dependent}
By reparameterization, we can accurately compute derivatives even in the presence of discontinuities. However, computing the boundary term in Equ.~\eqref{eq:reparameter_integral} requires searching for silhouette edges, 
which leads to a significant computational cost. Inspired by recent work \cite{Zhang:2020:PSDR}, we apply boundary path segmentation to avoid silhouette detection at every vertex. \xya{Essentially, the ray paths are created from the edges of the object controlled by $\theta$ expanding along two opposite directions to construct the path between Tx and Rx, as shown in Fig.~\ref{fig:path_space}(c).} We separate the boundary path into a transmission path \(\bar{p}^T\) and a receiver path \(\bar{p}^R\) at the discontinuity point \(p_K\): $\bar{p} = (p_t^T, \dots, p_0^T, p_0^R, \dots, p_r^R),$
where \((p_0^S, p_0^D) \in \mathcal{B}\times\Delta\mathcal{B}(p_{K-1})\). Then we can rewrite the boundary term of Equ.~\eqref{eq:reparameter_integral} as a combination of contributions from the source segment \(\hat{f}^S\), the boundary segment \(\hat{f}^B\) and the detection segment \(\hat{f}^D\):
\begin{equation}
\small
    \int_{\mathcal{B}}\int_{\Delta\mathcal{B}(p_{K-1})}\left(
    \int_{\Omega_0} \hat{f}^T\text{d}\mu^T
    \right)
    \hat{f}^B
    \left(
    \int_{\Omega_0} \hat{f}^R\text{d}\mu^R
    \right)
    \text{d}l(p_0^R)\text{d}A(p_0^T),
\label{eq:multi-direction-integral}
\end{equation}
where \(\hat{f}^T, \hat{f}^B, \hat{f}^R\) are all components of \(\hat{f}(p) V_{\partial}(p_K)\).

Through the multi-directional integral in Equ.~\eqref{eq:multi-direction-integral}, we can construct a boundary path as follows. Firstly, we sample the boundary segment \((p_0^T, p_0^R)\). Then we build the path from the source and the path towards the detector using 
bidirectional or unidirectional path sampling. 
This approach does not involve costly silhouette detection and therefore lowers the computational cost for the boundary term.

By combining this approach with reparameterization, we can bridge the gap between continuous and discontinuous changes in path space. 

\subsubsection{Differentiating Edge Diffraction}
\label{sec:dtd}

\xya{Simulating edge diffraction involves tracking wedges in the scene following the methods of the Uniform Theory of Diffraction (UTD). The method of differentiating edge diffraction can be treated as a combination of the methods proposed in Sec~\ref{sec:reparam} and \ref{sec:view_dependent}, as wedges are a subset of geometric edge and require tracking to construct diffraction path between Rx and Tx, as shown in Fig.~\ref{fig:path_space}(d).}
The diffracted field $E_d$ at a point can be expressed as $E_d = E_i D A(s) e^{-jks},$
where $E_i$ is the incident field, $D$ is the diffraction coefficient, $A(s)$ is the spreading factor, $k$ is the wave number, and $s$ is the distance from the diffraction point to the observation point.
\(\mathcal{E} \subseteq\partial\Omega\) denotes the edge points that have an edge diffraction effect. \(x_R\) is the position of the receiver. 
We can formulate the contribution of edge diffraction to 
the overall signal as:
\begin{equation}
\small
    h_D(t) = \int_{\mathcal{E}}E_d(\overline{xx_R})\text{d}A(x). 
\end{equation}
The differentiation of the diffraction process follows a similar approach including parameterization. Firstly, we map the edges to the reference surface \(\mathcal{B}\). Then we can calculate its derivative the same way as Equ.~\eqref{eq:reparameter_integral}. Since the edges \(\mathcal{E}\) are simple curves, the mapped points \(\mathcal{E}_0\) cannot be a plane and thus have no interior. Therefore, the derivative of the diffraction can be formulated as:
\begin{equation}
\small
    \frac{\partial h_D(t)}{\partial \theta} = \int_{\partial \mathcal{E}_0} \hat{E}_d(\overline{pp_R})V_{\partial}\text{d}l(p).
\end{equation}

\subsubsection{Monte Carlo Estimation of CIR Integrals}

In practical implementations, RF ray tracing simulators commonly estimate the CIR by integrating discrete propagation paths using the Monte Carlo method. \name simulates the CIR following the same approach, but must explicitly derive the gradients in this process. To this end, we note that the continuous integral of Equ.~\eqref{eq:step1} can be approximated by a sum over $N$ sampled paths:
\vspace{-3pt}
\begin{equation}
\small
h(t) \approx \frac{1}{N} \sum_{i=1}^N \hat{f}(p_i),
\end{equation}
\vspace{-3pt}
where $p_i$ are paths sampled from the path space $\Omega_0$. 

To estimate the derivative \wrt parameter $\theta$, we first apply the divergence theorem to convert the integral domain of the boundary term from \(\partial \Omega_0\) to \(\Omega_0\). The process can be formulated as:
\vspace{-3pt}
\begin{equation}
\tiny
\begin{aligned}
    \int_{\partial\Omega_0}\hat{f}(p)V_{\partial}(p_K)\text{d}\dot{\mu}(p)
    =& \sum_{N=1}^\infty\sum_{k=0}^{N-1}\int_{\mathcal{B}^{N+1}}\left[\nabla\cdot\left(\hat{f}_kV_{\partial}\right)\right](p_k)\text{d}\mu(p) \nonumber\\
    =& \int_{\Omega_0}\sum_{k=0}^{N-1}\left[\nabla\cdot\left(\hat{f}_kV_{\partial}\right)\right](p_k)\text{d}\mu(p),
\end{aligned}
\end{equation}
\vspace{-3pt}
Then we can calculate the derivative using Monte Carlo estimation:
\vspace{-3pt}
\begin{equation}
\small
\frac{\partial h(t)}{\partial \theta} \approx \frac{1}{N_I} \sum_{i=1}^{N_I} \left(\frac{\partial}{\partial \theta}\hat{f}(p_i) + \sum_{k=0}^{N-1} \left[\nabla\cdot\left(\hat{f}_kV_{\partial}\right)\right](p_k)\right).
\end{equation}
\vspace{-3pt}

This approach allows for efficient estimation of both the CIR and its derivatives. It is worth noting that in practical implementation, the multipath components of CIR are calculated separately, and hence the partial derivative $\frac{\partial \hat{\tau}}{\partial \theta}$, $\frac{\partial \hat{\alpha}}{\partial \theta}$,  $\frac{\partial \hat{\phi}}{\partial \theta}$ can be estimated via:

\vspace{-4mm}
\begin{equation}
\small
\left(\frac{\partial \tau_i}{\partial \theta},
\frac{\partial \phi_i}{\partial \theta},
\frac{\partial \alpha_i}{\partial \theta}\right)=
\frac{\partial}{\partial \theta} \hat{f}_y(p_i) + \hat{f}_y(p_i)V_\partial(p_{K,i}), \ y \in \{\tau, \phi, \alpha\}.
\end{equation}
\vspace{-4mm}

With this measure, the time-delay ($\tau$) and amplitude ($\alpha$) components of the CIR become differentiable. Consequently, we can backpropagate the gradients from the CIR to the 
DT scene ($\mathbf{\theta}$). \xya{Whereas the calculation of the partial derivatives is now complete, it may still suffer from local non-convexity issues (Sec.~\ref{sec:challenges}). We now introduce the surrogate models tailored to mitigate these challenges.}


==> Chapter/overview.tex <==
\section{System Overview}
\label{sec:design}

\newlength{\mylinewidth}
\setlength{\mylinewidth}{\}

Given a 3D scene parameterized by a continuous set $\theta$, which includes emitter/receiver, scene geometry, and material properties, \name aims to regenerate the received RF signals through differentiable ray tracing. Comparing the simulation and real measurement samples, it computes a scalar function (\eg, a loss function for optimization). The ultimate goal is to propagate gradients of this scalar with respect to all scene parameters $\theta$, so as to enable end-to-end differentiation across the simulation pipeline. 
This eventually forms a digital twin optimization framework (Fig.~\ref{fig:pull}), where the DT scene parameters $\theta$ gradually approach those of the physical twin upon convergence. 
 
\vspace{-5pt}
\subsection{Challenges and Observations}
\label{sec:challenges}

\noindent \textbf{Discontinuity.}
\label{sec:discontinuity}
A fundamental challenge in realizing physically correct differentiable RF ray tracing is handling edge discontinuities, where the edges of objects cause abrupt, non-smooth changes in the electromagnetic field. An object's edge can introduce such a discontinuity in two primary ways. \textit{First}, an edge inherent to an object's geometry, such as a corner, diffracts an incoming wave, scattering energy into regions not covered by direct or reflected paths. This diffracted field changes with extreme rapidity near the edge, effectively introducing a spatial singularity. \textit{Second}, from any given viewpoint, an edge defines the boundary of a shadow, separating an illuminated, line-of-sight region from an occluded one. Crossing this boundary causes a sharp drop in signal strength, resulting in a field with an extremely steep gradient. In both scenarios, these edge-induced effects introduce non-differentiable points into the modeled channel response, where the gradient is undefined. 
These non-differentiable points introduce significant complexities in modeling RF environments, particularly in inverse problem formulations and optimization scenarios.
  
\noindent \textbf{Non-Convexity from Wave Periodicity and Signal Processing.}
\label{sec:NonConvexity}
The non-convexity in RF propagation primarily stems from the periodic nature of electromagnetic waves and the complex multipath environments. This non-convexity introduces significant challenges in convergence for optimization algorithms and inverse problems. The periodicity of the phase is a fundamental source of non-convexity. Path length ambiguity arises from the phase difference $\Delta\phi$ between two points, given by $\Delta\phi = 2\pi(\Delta L/\lambda)$, where $\Delta L$ is the path length difference and $\lambda$ is the wavelength. Due to the $2\pi$ periodicity, multiple path lengths can result in the same phase difference, causing ambiguity in optimization problems. Furthermore, standing wave points occur at locations where waves from different paths interfere destructively, creating a deep fading region with very low field strength. These points introduce sharp valleys in the optimization landscape, preventing gradient-based methods from convergence.

Wideband radar waveforms such as frequency-modulated continuous wave (FMCW) or orthogonal frequency division modulation (OFDM) \cite{sit2011ofdm} leverage multiple frequency channels for sensing. Since electromagnetic waves with different wavelengths experience different phase shifts, Fourier analysis, \eg, discrete Fourier transforms (DFT), are commonly applied to the radar spectrum to separate reflections with different path lengths. However, with a finite number of discrete channel samples, Fourier analysis inevitably leads to \textit{sidelobes}~\cite{Oppenheim1998digital} whose peaks introduce another form of ambiguity in the parameter space. These sidelobes represent local minima that can be mistaken as true signal paths, creating additional non-convexity challenges in the optimization problem. \xya{High-resolution spectral estimation techniques such as MUSIC can suppress sidelobes, but they rely on eigenvalue decomposition of the sample covariance matrix (Appendix \ref{appendix:music}). While differentiable in principle, this operation suffers from extremely high gradient variance, making it unstable for gradient-based optimization.} Thus, neither DFT-based nor subspace-based methods can overcome the intrinsic non-convexity arising from wave periodicity and multipath interference.

